Cost-optimal Fleet Management Strategies for Solar-electric Autonomous Mobility-on-Demand Systems

This paper studies mobility systems that incorporate a substantial solar energy component, generated not only on the ground, but also through solar roofs installed on vehicles, directly covering a portion of their energy consumption. In particular, we focus on Solar-electric Autonomous Mobility-on-Demand systems, whereby solar-electric autonomous vehicles provide on-demand mobility, and optimize their operation in terms of serving passenger requests, charging and vehicle-to-grid (V2G) operations. We model this fleet management problem via directed acyclic graphs and parse it as a mixed-integer linear program that can be solved using off-the-shelf solvers. We showcase our framework in a case study of Gold Coast, Australia, analyzing the fleet's optimal operation while accounting for electricity price fluctuations resulting from a significant integration of solar power in the total energy mix. We demonstrate that using a solar-electric fleet can reduce the total cost of operation of the fleet by 10-15% compared to an electric-only counterpart. Finally, we show that for V2G operations using vehicles with a larger battery size can significantly lower the operational costs of the fleet, overcompensating its higher energy consumption by trading larger volumes of energy and even accruing profits.

==> Tools/acronyms.tex <==
\newcommand{\blueb}[1]{\textcolor{blue}{#1}}
\newcommand{\redb}[1]{\textcolor{red}{#1}}

\definecolor{lightblue}{rgb}{0.60784,0.76078,0.90196}
\definecolor{darkblue}{rgb}{0.26667,0.44706,0.76863}
\definecolor{lightgreen}{rgb}{0.66275,0.81569,0.55686}
\definecolor{darkgreen}{rgb}{0.43922,0.67843,0.27843}
\definecolor{orange}{rgb}{0.92941,0.49020,0.19216}
\definecolor{yellow}{rgb}{1.00000,0.75294,0.00000}
\definecolor{grey}{rgb}{0.64706,0.64706,0.64706}
\definecolor{purple}{rgb}{0.51373,0.23529,0.04706}
% a
\newacronym{abk:amod}{AMoD}{Autonomous Mobility-on-Demand}
\newacronym{abk:iamod}{I-AMoD}{intermodal \gls{abk:amod}}
% b
\newacronym{abk:bpr}{BPR}{the Bureau of Public Roads}
% c
\newacronym{abk:ca}{CA}{congestion-aware}
\newacronym{abk:cara}{CARS}{congestion-aware routing scheme}
\newacronym{abk:cepamods}{CEPAMoDS}{Convolutional Energy Predicting AMoD Scheduler}
\newacronym{abk:cs}{CS}{charging station}
% d
% e
% f
\newacronym{abk:ffcs}{FFCS}{free floating car sharing systems}
% g
\newacronym{abk:ghg}{GHG}{greenhouse gas}
% h
% i
% j
% k
\newacronym{abk:kpi}{KPIs}{Key Performance Indicators}
% l
% m
\newacronym{abk:mcfp}{MCFP}{multi-commodity flow problem}
\newacronym{abk:milp}{MILP}{mixed-integer linear program}
% n
% o
% p
% q
% r
% s
\newacronym{abk:spp}{SPP}{shortest path problem}
\newacronym{abk:kdspp}{k-dSPP}{k-disjoint \gls{abk:spp}}
\newacronym{abk:soc}{SoC}{state of charge}
% t
% u
% v
\newacronym{abk:vrp}{VRP}{vehicle routing problem}
\newacronym{abk:v2g}{V2G}{vehicle-to-grid}
% w
% x
% y
% z	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commands
% \newcommand{}{}
%-Large-Arabic-------------------------------------------------------------------------------
% A
%\newcommand{}{A}
\newcommand{\eqMatrix}{\mathbf{A}}
% B
%\newcommand{}{B}
% C
%\newcommand{}{C}
% D
%\newcommand{}{D}
\newcommand{\ineqMatrix}{\mathbf{D}}
% E
%\newcommand{}{E}
% F
%\newcommand{}{F}
\newcommand{\BPR}{F_\mathrm{BPR}}
% G
%\newcommand{}{G}
% H
%\newcommand{}{H}
% I
%\newcommand{}{I}
% J
%\newcommand{}{J}
% K
%\newcommand{}{K}
% L
%\newcommand{}{L}
% M
%\newcommand{}{M}
% N
%\newcommand{}{N}
% O
%\newcommand{}{O}
% P
%\newcommand{}{P}
\newcommand{\Pru}{P_\mathrm{rush}}
\newcommand{\Pch}{P_\mathrm{chill}}
% Q
%\newcommand{}{Q}
% R
%\newcommand{}{R}
% S
%\newcommand{}{S}
\newcommand{\source}{S_{o}}
\newcommand{\sink}{S_{d}}
% T
%\newcommand{}{T}
\newcommand{\resCost}{T^{\mathrm{c}}}
\newcommand{\resPred}{T^{\mathrm{p}}}
% U
%\newcommand{}{U}
% V
%\newcommand{}{V}
\newcommand{\vTime}{V_\mathrm{T}}
\newcommand{\vDistR}{V_\mathrm{D}}
\newcommand{\vDistS}{V_\mathrm{D,P}}
\newcommand{\vEnergy}{V_\mathrm{E}}
\newcommand{\vCO}{V_{\mathrm{CO}_2}}
\newcommand{\vQuadratic}{V_\mathrm{Q}}
% W
%\newcommand{}{W}
% X
%\newcommand{}{X}
% Y
%\newcommand{}{Y}
% Z
%\newcommand{}{Z}
%-Small-Arabic-------------------------------------------------------------------------------
% a
%\newcommand{}{a}
% b
%\newcommand{}{b}
\newcommand{\eqRHS}{\mathbf{b}}
% c
%\newcommand{}{c}
\newcommand{\capacity}{c}
\newcommand{\capacityRoad}{c^{\mathrm{R}}}
\newcommand{\capacityRoadTh}{c^{\mathrm{R,th}}}
\newcommand{\capacityPublic}{c^{\mathrm{P}}}
\newcommand{\cost}{J}
\newcommand{\costQ}{J_\mathrm{Q}}
\newcommand{\costM}{J_\mathrm{M}}
\newcommand{\costE}{J_{\mathrm{CO}_2}}
\newcommand{\transpCoeff}{\mathbf{c}^\top}
% d
%\newcommand{}{d}
\newcommand{\destination}{d}
\newcommand{\ineqRHS}{\mathbf{d}}
% e
%\newcommand{}{e}
\newcommand{\energyR}{e_{ij}}
\newcommand{\sC}{s_{\mathrm{CO}_2}}
\newcommand{\energyS}{e_{\mathrm{S},ij}}
\newcommand{\energySperpaxmile}{\bar{e}_{\mathrm{P}}}
% f
%\newcommand{}{f}
\newcommand{\flow}[2]{f_m\left(#1,#2\right)}
\newcommand{\flowTot}[2]{f\left(#1,#2\right)}
\newcommand{\flowzero}[2]{f_m\left(#1,#2\right)}
\newcommand{\flowReba}[2]{f_0\left(#1,#2\right)}
% g
%\newcommand{}{g}
% h
%\newcommand{}{h}
% i
%\newcommand{}{i}
% j
%\newcommand{}{j}
% k
%\newcommand{}{k}
% l
%\newcommand{}{l}
% m
%\newcommand{}{m}
% n
%\newcommand{}{n}
% o
%\newcommand{}{o}
\newcommand{\origin}{o}
% p
%\newcommand{}{p}
\newcommand{\route}{p}
\newcommand{\pSubway}{p_\mathrm{P}(i,j)}
\newcommand{\pRoad}{p_\mathrm{R}(i,j)}
\newcommand{\pOrigin}[1]{p_\mathrm{O}\left(#1\right)}
\newcommand{\pDest}[1]{p_\mathrm{D}\left(#1\right)}
% q
%\newcommand{}{q}
% r
%\newcommand{}{r}
\newcommand{\request}{r}
\newcommand{\weight}{r_\mathrm{E}}
% s
%\newcommand{}{s}
% t
%\newcommand{}{t}
\newcommand{\traveltime}{t}
\newcommand{\traveltimeNom}{t^N}
\newcommand{\traveltimezero}{t^0}
\newcommand{\tRoad}{\tau_\mathrm{R}(i,j)}
% u
%\newcommand{}{u}
\newcommand{\usageRoad}{u^\mathrm{R}}
% v
%\newcommand{}{v}
% w
%\newcommand{}{w}
% x
%\newcommand{}{x}
\newcommand{\decVec}{\mathbf{x}}
% y
%\newcommand{}{y}
% z
%\newcommand{}{z}
%-Large-Calligraphic-------------------------------------------------------------------------
% A
%\newcommand{}{\mathcal{A}}
\newcommand{\setOfArcs}{\mathcal{A}}
\newcommand{\setOfArcsRoad}{\mathcal{A}_{\mathrm{R}}}
\newcommand{\setOfArcsSubway}{\mathcal{A}_{\mathrm{P}}}
\newcommand{\setOfArcsPedestrian}{\mathcal{A}_{\mathrm{W}}}
\newcommand{\setOfArcsCommute}{\mathcal{A}_{\mathrm{C}}}
%\newcommand{\setOfArcsSP}{\mathcal{A}_{\mathrm{SP}}}
% B
%\newcommand{}{\mathcal{B}}
% C
%\newcommand{}{\mathcal{C}}
% D
%\newcommand{}{\mathcal{D}}
% E
%\newcommand{}{\mathcal{E}}
%\newcommand{\setOfArcs}{\mathcal{E}}
%\newcommand{\setOfArcsRoad}{\mathcal{E}_{\mathrm{R}}}
%\newcommand{\setOfArcsPublic}{\mathcal{E}_{\mathrm{P}}}
%\newcommand{\setOfArcsCommute}{\mathcal{E}_{\mathrm{C }}}
% F
%\newcommand{}{\mathcal{F}}
% G
%\newcommand{}{\mathcal{G}}
\newcommand{\Graph}{\mathcal{G}}
\newcommand{\GraphRoad}{\mathcal{G}_\mathrm{R}}
\newcommand{\GraphSubway}{\mathcal{G}_\mathrm{P}}
\newcommand{\GraphPedestrian}{\mathcal{G}_\mathrm{W}}
% H
%\newcommand{}{\mathcal{H}}
% I
%\newcommand{}{\mathcal{I}}
% J
%\newcommand{}{\mathcal{J}}
% K
%\newcommand{}{\mathcal{K}}
\newcommand{\setOfModes}{\mathcal{K}}
% L
%\newcommand{}{\mathcal{L}}
% M
%\newcommand{}{\mathcal{M}}
\newcommand{\setOfRequestsNumber}{\mathcal{M}}
% N
%\newcommand{}{\mathcal{N}}
% O
%\newcommand{}{\mathcal{O}}
% P
%\newcommand{}{\mathcal{P}}
\newcommand{\pathSet}{\mathcal{P}}
% Q
%\newcommand{}{\mathcal{Q}}
% R
%\newcommand{}{\mathcal{R}}
\newcommand{\setOfRequests}{\mathcal{R}}
% S
%\newcommand{}{\mathcal{S}}
\newcommand{\subSet}{\mathcal{S}}
% T
%\newcommand{}{\mathcal{T}}
% U
%\newcommand{}{\mathcal{U}}
% V
%\newcommand{}{\mathcal{V}}
\newcommand{\setOfVertices}{\mathcal{V}}
\newcommand{\setOfVerticesRoad}{\mathcal{V}_{\mathrm{R}}}
\newcommand{\setOfVerticesSubway}{\mathcal{V}_{\mathrm{P}}}
\newcommand{\setOfVerticesPedestrian}{\mathcal{V}_{\mathrm{W}}}
% W
%\newcommand{}{\mathcal{W}}
% X
%\newcommand{}{\mathcal{X}}
% Y
%\newcommand{}{\mathcal{Y}}
% Z
%\newcommand{}{\mathcal{Z}}
%-Large-Scr-------------------------------------------------------------------------
% A
%\newcommand{}{\mathscr{A}}
\newcommand{\setOfMultiArcs}{\mathscr{A}}
% B
%\newcommand{}{\mathscr{B}}
% C
%\newcommand{}{\mathscr{C}}
% D
%\newcommand{}{\mathscr{D}}
% E
%\newcommand{}{\mathscr{E}}
% F
%\newcommand{}{\mathscr{F}}
% G
%\newcommand{}{\mathscr{G}}
\newcommand{\multigraph}{\mathscr{G}}
\newcommand{\multigraphC}{\mathscr{G}'}
% H
%\newcommand{}{\mathscr{H}}
% I
%\newcommand{}{\mathscr{I}}
% J
%\newcommand{}{\mathscr{J}}
% K
%\newcommand{}{\mathscr{K}}
% L
%\newcommand{}{\mathscr{L}}
% M
%\newcommand{}{\mathscr{M}}
% N
%\newcommand{}{\mathscr{N}}
% O
%\newcommand{}{\mathscr{O}}
% P
%\newcommand{}{\mathscr{P}}
\newcommand{\setOfArcsIndex}{\mathscr{P}}
% Q
%\newcommand{}{\mathscr{Q}}
% R
%\newcommand{}{\mathscr{R}}
% S
%\newcommand{}{\mathscr{S}}
% T
%\newcommand{}{\mathscr{T}}
% U
%\newcommand{}{\mathscr{U}}
% V
%\newcommand{}{\mathscr{V}}
% W
%\newcommand{}{\mathscr{W}}
% X
\newcommand{\decvecSet}{\mathcal{X}}
% Y
%\newcommand{}{\mathscr{Y}}
% Z
%\newcommand{}{\mathscr{Z}}
\newcommand{\setOfMultiarcIndex}{\mathscr{Z}}
%-Large-Greek--------------------------------------------------------------------------------
% Alpha
%\newcommand{}{A}
% Beta
%\newcommand{}{B}
% Gamma
%\newcommand{}{\Gamma}\\
\newcommand{\neighborOne}{\Gamma}
% Delta
%\newcommand{}{\Delta}
% Epsilon
%\newcommand{}{E}
% Zeta
%\newcommand{}{Z}
% Eta
%\newcommand{}{H}
% Theta
%\newcommand{}{\Theta}
% Iota
%\newcommand{}{I}
% Kappa
%\newcommand{}{K}
% Lambda
%\newcommand{}{\Lambda}
% Mu
%\newcommand{}{M}
% Nu
%\newcommand{}{N}
% Xi
%\newcommand{}{\Xi}
% Omicron
%\newcommand{}{O}
% Pi
%\newcommand{}{\Pi}
% Rho
%\newcommand{}{P}
% Sigma
%\newcommand{}{\Sigma}
% Tau
%\newcommand{}{T}
% Upsilon
%\newcommand{}{\Upsilon}
% Phi
%\newcommand{}{\Phi}
% Chi
%\newcommand{}{X}
% Psi
%\newcommand{}{\Psi}
% Omega
%\newcommand{}{\Omega}
%-Small-Greek--------------------------------------------------------------------------------
% alpha
%\newcommand{}{\alpha}
\newcommand{\requestrate}{\alpha}
% beta
%\newcommand{}{\beta}
% gamma
%\newcommand{}{\gamma}
% delta
%\newcommand{}{\delta}
\newcommand{\cutsetSucc}[1]{\delta^{\text{+}}\left(#1\right)}
\newcommand{\cutsetPred}[1]{\delta^{\text{-}}\left(#1\right)}
% epsilon
%\newcommand{\slack}{\varepsilon}
\newcommand{\slack}[2]{\varepsilon\left(#1,#2\right)}
% zeta
%\newcommand{}{\zeta}
% eta
%\newcommand{}{\eta}
% theta
%\newcommand{}{\vartheta}
% iota
%\newcommand{}{\iota}
\newcommand{\iteration}{\iota}
% kappa
%\newcommand{}{\kappa}
% lambda
%\newcommand{}{\lambda}
\newcommand{\lgeq}{\mathbf{\lambda}}
\newcommand{\dualEq}{\lambda_{ij}}
\newcommand{\dualCust}{\lambda_\mathrm{C}}
\newcommand{\dualVeh}{\lambda_\mathrm{R}}
\newcommand{\dualCustTilde}{\tilde{\lambda}_\mathrm{C}}
\newcommand{\dualVehTilde}{\tilde{\lambda}_\mathrm{R}}
% mu
%\newcommand{}{\mu}
\newcommand{\dualCR}{\mu_\mathrm{cR}}
\newcommand{\lgineq}{\mathbf{\mu}}
\newcommand{\dualIneq}{\mu}
\newcommand{\dualcR}{\mu_\mathrm{cR}}
\newcommand{\dualcS}{\mu_\mathrm{cP}}
% nu
%\newcommand{}{\nu}
% xi
%\newcommand{}{\xi}
% omicron
%\newcommand{}{o}
% pi
%\newcommand{}{\pi}
% rho
%\newcommand{}{\rho}
% sigma
%\newcommand{}{\sigma}
% tau
%\newcommand{}{\tau}
% upsilon
%\newcommand{}{\upsilon}
% phi
%\newcommand{}{\phi}
% chi
%\newcommand{}{\chi}
% psi
%\newcommand{}{\psi}
% omega
%\newcommand{}{\omega}
%-Other-------------------------------------------------------------------
\newcommand{\arc}{(i,j)}
\newcommand{\multiarc}{(i,j,z)}
\newcommand{\bool}[1]{\mathds{1}_{#1}}
